The Zero Resource Speech Challenge 2020: Discovering discrete subword and word units

We present the Zero Resource Speech Challenge 2020, which aims at learning speech representations from raw audio signals without any labels. It combines the data sets and metrics from two previous benchmarks (2017 and 2019) and features two tasks which tap into two levels of speech representation. The first task is to discover low bit-rate subword representations that optimize the quality of speech synthesis; the second one is to discover word-like units from unsegmented raw speech. We present the results of the twenty submitted models and discuss the implications of the main findings for unsupervised speech learning.

==> reviews.tex <==
============================================================================
                            REVIEWER #1
============================================================================

Detailed Comments for Authors
---------------------------------------------------------------------------
-- Detailed Review --
This paper describes the outcome of the ZeroSpeech 2020 challenge. The paper details the challenge task, data, submitted models, and experimental results. The goals of the challenge this year were twofold: Track 1 involved learning training models to learn a small number of discrete sub-word speech units for performing voice conversion. Track 2 involved segmentation and clustering of the speech signal for the purpose of discovering word-like units. Both tasks supply common training/development data as well as separate evaluation data from a “surprise” language(s) that is different from the training data. The paper provides a very thorough comparison of the experimental results from 20 submitted systems, and in doing so establishes a current benchmark for the field of unsupervised speech processing as a whole.

-- Key Strength of the paper --
This paper summarizes the results obtained by the 20 submissions to the ZeroSpeech 2020 Challenge. Many of the submissions utilize novel modeling techniques or novel combinations of existing techniques for unsupervised learning of speech. Therefore, this paper pushes the state of the art in this field by providing a shared evaluation benchmark for these systems.

-- Main Weakness of the paper --
I have a few suggestions/comments for the authors:

Page 3, second column, top paragraph: “We restrict both sets to words between three and twenty segments long.” It is not clear from the writing in this section what "segment" refers to.

Section 2.1:  For the ABX task, when computing the features for a given triphone segment, is the input given to each system only the waveform segment corresponding to the triphone? Or does a system have access to the acoustic context before/after the triphone segment? If the former is the case, I wonder if there is too much constraint/burden placed on the models, because they would not have the opportunity to model co-articulation effects outside of the triphone, perform implicit speaker normalization, model phonotactics, etc. which all could take advantage of longer term dependencies in the signal. An alternative approach might be to ask the system to compute time-aligned features/units at the utterance level (or longer) and then perform the ABX comparison with the time-aligned features/units.
---------------------------------------------------------------------------


Explanation - Quality of the paper
---------------------------------------------------------------------------
-- Novelty/Originality --
The paper benchmarks many novel approaches for unsupervised speech processing on the ZeroSpeech 2020 challenge data and tasks.

-- Technical Correctness -- 
The paper is technically correct as far as I can tell.

-- Clarity of Presentation -- 
The paper is very clearly written and easy to understand.

-- Quality of References -- 
The references are thorough.

-- Reproducibility --
The data and software evaluation framework used in the ZeroSpeech 2020 challenge is open source, and many of the submissions also make their code and models publicly available.
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #2
============================================================================

Detailed Comments for Authors
---------------------------------------------------------------------------
Hard to "review" a Challenge summary paper.

Everything is pretty well written.

Fig.1 is very much appreciated, in order to put this Challenge in its historical
context, and to get the meaning at a glance.

The 2D plots of Fig.2 are great too. I didn't get the reason for pairing
some measures and not some others though.
---------------------------------------------------------------------------


Explanation - Quality of the paper
---------------------------------------------------------------------------
Hard to "review" a Challenge summary paper.

Everything is pretty well written.

Fig.1 is very much appreciated, in order to put this Challenge in its historical
context, and to get the meaning at a glance.

The 2D plots of Fig.2 are great too. I didn't get the reason for pairing
some measures and not some others though.
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #3
============================================================================

Detailed Comments for Authors
---------------------------------------------------------------------------
This paper describes the main characteristics of the Zero Resource Speech Challenge 2020, its motivation, the two tasks (unsupervised unit discovery for speech synthesis, and spoken term discovery and segmentation), the conditions of participation, the datasets, metrics and baseline systems. Then, it presents an overview of participation and the results obtained in the two tasks, with more emphasis on the first one. The series of ZeroSpeech evaluations is one the most ambitious and interesting initiatives in the field of speech technology. It fosters new unsupervised approaches to speech modeling, with small but consistent improvements every year. I am skeptical about the final goal of completely removing the need for supervision because human communication is based on symbols and there should always be some connection (at some point) between those arbitrary symbols and the acoustic (subword or word-level) units automatically discovered. But aside from this philosophical con!
 cern, I enthusiastically support the initiative and am curious about the new advancements it will give rise.

I find them difficult to understand at first sight the graphs of Figure 2. I understand that such a lot of information is difficult to present in such a small space; I would rather focus on just two or three aspects of the evaluation, e.g. quality and bitrate, on separate tracks.

The writing is easy and clear but I found two typos: a repetition of "more than" at the end of the penultimate paragraph of section 2.2, and the word "of" that must be deleted in the middle of the last paragraph of section 2.2 ("The parameters stayed the same...").
---------------------------------------------------------------------------


Explanation - Quality of the paper
---------------------------------------------------------------------------
This paper would probably require twice or three times the space given to a standard Interspeech paper to fully account for the preparation of data, to describe and discuss the design decisions, data preparation, definition of metrics, etc. This is just an overview of the evaluation, but it contains the most important elements of it: its historical motivation and the ultimate goal of removing supervision from speech technology (about which I am skeptical), a brief description of the tasks, the datasets and metrics used in each case, and finally a very compact (and hardly understandable) account of the performance attained by the submitted systems. Given the limited space, I would have rather focused on two separate analyses: ABX error and bitrate, instead of the wider but cryptic analysis provided with Figure 2. Congratulations to the organizers for another successful edition of ZeroSpeech.
---------------------------------------------------------------------------


